Mapping the Join Calculus to Heterogeneous Hardware

As modern architectures introduce additional heterogeneity and parallelism, we look for ways to deal with this that do not involve specialising software to every platform. In this paper, we take the Join Calculus, an elegant model for concurrent computation, and show how it can be mapped to an architecture by a Cartesian-product-style construction, thereby making use of the calculus' inherent non-determinism to encode placement choices. This unifies the concepts of placement and scheduling into a single task.

==> eptcsdata.tex <==
\providecommand{\firstpage}{7}
\providecommand{\publicationstatus}{S. J. Gay and P. H. Kelly (Eds.): Programming Language Approaches to\\
Concurrency- and Communication-cEntric Software (PLACES 2012)\\
EPTCS 109, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.109.2}{10.4204/EPTCS.109.2}}

